Deep Crowd-Flow Prediction in Built Environments

Predicting the behavior of crowds in complex environments is a key requirement in a multitude of application areas, including crowd and disaster management, architectural design, and urban planning. Given a crowd's immediate state, current approaches simulate crowd movement to arrive at a future state. However, most applications require the ability to predict hundreds of possible simulation outcomes (e.g., under different environment and crowd situations) at real-time rates, for which these approaches are prohibitively expensive. In this paper, we propose an approach to instantly predict the long-term flow of crowds in arbitrarily large, realistic environments. Central to our approach is a novel CAGE representation consisting of Capacity, Agent, Goal, and Environment-oriented information, which efficiently encodes and decodes crowd scenarios into compact, fixed-size representations that are environmentally lossless. We present a framework to facilitate the accurate and efficient prediction of crowd flow in never-before-seen crowd scenarios. We conduct a series of experiments to evaluate the efficacy of our approach and showcase positive results.

==> Tex/1contributions.tex <==
\begin{itemize}
    \item We formalize an input representation consisting of \textbf{C}apacity-, \textbf{A}gent-, \textbf{G}oal-, and \textbf{E}nvironment-oriented information (\texttt{CAGE}) that is well-suited for crowd density prediction and its future developments.
    \item We describe a novel generator for the floorplans of built environments that provides a representative sample based on the typologies of modern architecture.
    \item \red{We evaluate the capability of a deep convolutional encoder-decoder network to satisfy the key requirements crowd density prediction.} \mk{be more specific of the type of architecture, why it was chosen etc}
    \item We present a predictor that --in combination with the \CAGE representation and the floorplan generator-- is not limited to a fixed-size environments. \mk{there is absolutely no mention of your method to support any sized environments -- the technical contribution is *NOT* what you can do, but how you can do it}
\end{itemize}
